Privacy-Preserving Spam Filtering using Functional Encryption

Traditional spam classification requires the end-user to reveal the content of its received email to the spam classifier which violates the privacy. Spam classification over encrypted emails enables the classifier to classify spam email without accessing the email, hence protects the privacy of email content. In this paper, we construct a spam classification framework that enables the classification of encrypted emails. Our classification model is based on a neural network with a quadratic network part and a multi-layer perception network part. The quadratic network architecture is compatible with the operation of an existing quadratic functional encryption scheme that enables our classification to predict the label of encrypted emails without revealing the associated plain-text email. The evaluation results on real-world spam datasets indicate that our proposed spam classification model achieves an accuracy of over 96%.

==> Privacy_attack_data_leakage.tex <==
\section{Data Leakage in the Plain-text Network}
In this section, we discuss the possibility of adversary to leverage the trained model's output which results in data leakage. 
The adversary still can leverage the decryption output of the FE to gain private information. We will analyse how likely the adversary could profit from this. 
Then, we examine possible countermeasures to this attack. Specifically, we will use methods proposed by Ryffel et. al. and examine its efficiency in reduce the sensitivity of the decrypted output with text classification.

\subsection{Data Leakage}
In the email spam filtering use case, the output of the FE scheme represents the likelihood of whether an email is spam or normal. The adversary can use the output to gain other information such as the email category. For example, they can know if the email contains finance information, or employee information. To do that, the attacker builds a new neural network model and uses the output of the FE scheme as the model feature to train the model. 

In practice, the attack could be that an adversary compromised the email server and has access to the output of the encrypted model (private network). Besides, the adversary has an amount of history plaintext emails which could be used by the adversary to train a new neural network model to classify the email category. In organization, the email contains indirect information which can be leveraged to reveal the critical financial activities. For example, if the number of emails between two organizations is increasing, that can imply that two organizations could cooperate on some events recently. The adversary could combine the information which he gets from the data leakage in the email server and the public news to predict the private activities are going to be performed by the organizations. In some cases, the information should be valuable which can impact the organization’s stock value. Figure 18 shows the framework of the attack. 

% \subsection{Collateral Learning Attack}
The emails dataset does not contain two types of labels. Thus, we cannot simulate the private prediction. In this paper, we simulate the possible attack on news dataset which has two independent data labels. The main task of the machine learning model is to predict the public label, i.e., news source $[CNN, FOX]$. The adversary's task is to predict the private data label, i.e., news category $[technology,\ health,\ travel]$. 
Figure 19 shows the model architecture used in the data leakage issue analysing.

The original model consists of two parts, the FE scheme encrypted model (private network) and an unencrypting mode (plaintext network) used to enhance the model accuracy. Although the attacker could not reveal the plaintext news in the encrypted model, if it could obtain the output of the encrypted model (model parameters of output layer of the private network), it can feed the output model parameters to adversary model in order to classify the dataset and extract additional information from encrypted data. The original model using the loss function:
\[Loss(org) = Minimize \ L_{pub} (\theta(FE), \theta(unenc))\]

The attacker uses below loss function to gain additional information:
\[Loss(atk) = Minimize \ L_{pri} (frozen(\theta(FE)), \theta(adv))\]
Figure \ref{fig:data_leakage} shows the accuracy of the private tasks which are triggered by the adversary to gain private data label. In this case, the private data label is news category.

The average accuracy of the private tasks is around 68.89\% in a three classes of text classification model prediction. The adversary can easily leverage the data leakage in the FE scheme to gain additional information.

\begin{figure}[ht!]
\centering
\includegraphics[width=\linewidth]{figures/Data_Leakage.pdf}
\caption{Data leakage issue, x-axis is the order of an experiment (news dataset)  \label{fig:data_leakage}} 
\end{figure}

\subsection{Collateral Learning}
The goal is to keep the accuracy of the main task while reduce the accuracy of the private task. When building the collateral training model, the label for the private prediction task should be known at first. Figure 21 shows the framework of the collateral training.

The framework of the collateral training is fork-like architecture. Both the public tasks enhance model and the private adversary model use the output of the FE output (private network) as their inputs but with different goals. In the collateral training, the public enhance model and the adversary mode are frozen, the FE scheme model is retrained using the combination loss function:
\begin{equation}
\begin{aligned}
Loss (coll) = & Minimize \{ L_{pub} (\theta(FE), freeze(\theta(pub))) \\
& - \alpha L_{pri} (\theta(FE), freeze(\theta(adv))) \}   
\end{aligned}
\end{equation}


Figure 22 shows the model summary of the collateral training. 

The collateral loss function has two parts: $L_{pub} (\theta(FE), freeze(\theta(pub))$ and $\alpha L_{pri} (\theta(FE), freeze(\theta(adv)))$. To get the minimum loss function, the first part should be as less as possible, and the second part should be large as much as possible. In the model summary, the input layer, second layer, lambda and Q output layer composite the equivalent encrypted FE model, $\theta(FE)$. The first part of the collateral loss function has FE scheme model and public enhanced model, six layers and pub output layer in the model summary. The second part of the collateral loss function makes of encrypted FE model and the adversary model which has third layer, forth layer, fifth layer, test1 and pri output layer. Regarding the collateral loss function, the accuracy for the public tasks increases while the accuracy of the private tasks decrease. After the collateral training, the FE model should  keep the original accuracy of the public task and contain less information for the private training. 

After we have the new FE model, the final step is to use the new FE model to build the new public model and adversary model to see if the FE effectively reduce the data leakage issue which is the recovery phase.
After the collateral training, a new $\theta(FE)$ is generated. Compared to the original $\theta(FE)$, it should keep the main task accuracy and sharply reduce the adversary tasks accuracy. To approve that, a new public enhanced model and the adversary model will be trained based on the output of the new $\theta(FE)$. Figure 23 and Figure 24 shows the public enhanced model and adversary model used in the recover stage.

In the combination loss function of the collateral training, the coefficients $\alpha$ is chosen to control the penalty term as the regularization used in the machine learning. The larger $\alpha$ is, the impact of the adversary training are consider in the new FE encrypted model training process. Figure 25 shows the impact of $\alpha$ on the accuracy of the public and adversary training.

From the figure 25, it shows the larger $\alpha$ is, the less accurate both tasks are. Comparing the impact of $\alpha$ on the main and private tasks, the accuracy of main task drops with a smaller amount compared to the accuracy of the private tasks. Another fact is when $\alpha > 1$ , the impact of $\alpha$ has slight impact on the neural network model. For the news dataset, we can see the $\alpha =1$ is the tuning point for the collateral learning. The model owner should set $\alpha =1$ during the collateral training to gain the new FE model because the new FE model using $\alpha =1$ is more efficient in keeping the main tasks performance and remediate the data leakage issue in the FE scheme. 

\begin{figure}[ht!]
\centering
\includegraphics[width=\linewidth]{figures/Alpha_Impact.pdf}
\caption{Impact of $\alpha$ on collateral learning accuracy \label{fig:impact_alpha}} 
\end{figure}



==> System_Model.tex <==
% \section{Spam Filtering Framework}
% This section first presents our machine learning model using the quadratic functional encryption for text classification in general. We then our proposed the spam filtering framework. 

% \subsection{Neural Network Model}
% The quadratic functional encryption scheme is equivalent to a one-hidden layer quadratic network. At the beginning, a pair $(\vec{X}, \vec{Y})$ represent the feature of one data. In our model, $\vec{X}=\ \vec{Y} = (x_1, x_2, \dots, x_n)$, $n$ is the length of feature after feature selection. In other use case, user can use arbitrary $(\vec{X},\vec{Y})$ to form the polynomial decision boundary they want to use in the encryption model. Although functional encryption scheme output $\vec{X} \dot \vec{F} \dot \vec{Y}$ is same as the output of one fully connected linear layer, the large size of the  $\vec{X}$ and $\vec{Y}$ cause encryption and decryption process consume huge compute resource and require long time. This problem is specially concern in text classification task because the feature of the data generally is the vocabulary dictionary size. After using information gain to select the feature, other measure is needed to further reduce the feature length to release the compute burden during encryption and decryption process.
% To reduce the calculation time in encryption, using the linear homomorphism feature of the functional encryption scheme is an efficient way. Originally, the secrete key $msk$ $(\vec{S},\vec{T})$ can encrypt the plaintext $(\vec{X},\ \vec{Y})$. Due to the linear hommomorphism, the $msk$ $(\vec{U} \vec{S}, \vec{V} \vec{T})$ can encrypt the plaintext $(\vec{U} \vec{X} , \vec{V} \vec{Y})$ where $\vec{U},\vec{V} \in \mathbb{Z}_p^{d\times n}$. After the linear conversion, the feature size change from $n$ to $d$. It efficiently reduce the compute resource needed for the encryption. Another way to accelerate encryption is to use caching. In the last step of the decryption, it computes discrete logarithms of group elements. The discrete logarithms does not associate with the decryption key and ciphertext, so it can be pre-calculated and cached to accelerate the decryption time. As the discrete logarithms is the most expensive step, pre-calculating and caching can reduce the time dramatically.
% whole encryption process forms a degree two polynomial network with one hidden layer. However, this simple model may not efficient enough to predict the spam at high accuracy. To enhance the accuracy, after the encryption process, an unencrypted network can be added after the encryption model. In the unencrypted network, it takes the output layer of the encryption model as its input and additional layers and activation function to improve the prediction accuracy. Figure 11 shows the architecture of the entire model.

 
% Figure 11 shows structure of the neural network model. The model should be treated as a whole to classify the text. The output of the encryption part of the model do not need to equal to the number of the data class. It can be regarded as one of the hidden layers in the whole neural network model. However, the larger the size of the output, the more data leakage occurs. 


% \subsection{Email Spam Filtering Framework}
% There are two phases in the process of using privacy-preserving spam filtering framework. The first phase is model training stage. In this stage, neural network model is trained based on the plaintext training data. Encryption does not occur in the training. After the training stage, both encrypted part and unencrypted part of the model weight and bias are confirmed. The weight of the encrypted part model will be used to generate the decryption key, and the weight of the unencrypted part model will be used on prediction stage. 
% Second stage is the prediction phase, the encrypted email data transport to the email server, and the email server decrypts the content. The output of the decryption is same as the output of plaintext data go through the encrypted model part. Because of that, the next step is feeding the decrypted data into the unencrypted model layers to get the output layer of the model. Figure 13 shows the data flow of the prediction.

% The framework of the email prediction process includes five components, sender user agent, sender mail server agent, receiver mail server agent, receiver user agent and spam filter service provide.
% Sender user agent is installed on the email sender’s computer, it is responsible to represent the text email content into document-term-matrix vector, encrypt the email using the PK, then send the vector, PK and MSK to sender mail server agent. Next component is sender mail server agent, it works on SMTP server to send the encrypted email and PK to receiver mail server agent. The third component receiver email server agent acts as an IMAP server to receive email from SMTP server followed by generating the DK based on MSK, and use the DK, model weight and bias to decrypt the email and do the prediction. Given that, the receiver email server need MSK, pre-trained model and the independent discrete number database for decryption and prediction. After knowing the email type, the receiver mail server agent forwards the email to receiver’s user agent component installed on receiver’s local computer. In this process, a Spam filter service provider is necessary. It is the third-part software provider who provide the spam filter service or plugins to other components. It provides other agent spam filtering pre-trained model, encryption decryption algorithm, document-term-matrix, key generation algorithm and the pre-compute discrete number database. Figure 14 shows the data flow from each component.

% At the beginning, process one and process two in the figure 11 is initiated. The Spam filter server send the sender user agent the MSK, PK, DK generation algorithm, document-term-matrix, the functional encryption algorithm and pre-trained model weight and bias. After the initiation, both sender and receiver are ready to predict the encrypted email. In the process three, the sender write the email and represent it through document-term-matrix vector and encrypt the original email using MK and PK, then it send the vectors and the original text email to the sender email server (process 4) followed by forwarding the encrypted vector and text email to the receiver email server agent (process 5). In process 6, the receiver mail server agent will use the received model and decryption key to decrypt the vector and predict the email type. In the whole prediction process, the email server agent never touches the text email. Given that, the user’s privacy is not revealed to the server in the whole process. However, users can leverage the server to filter the spam emails.


